Ignorance is Almost Bliss: Near-Optimal Stochastic Matching With Few Queries

The stochastic matching problem deals with finding a maximum matching in a graph whose edges are unknown but can be accessed via queries. This is a special case of stochastic $k$-set packing, where the problem is to find a maximum packing of sets, each of which exists with some probability. In this paper, we provide edge and set query algorithms for these two problems, respectively, that provably achieve some fraction of the omniscient optimal solution. Our main theoretical result for the stochastic matching (i.e., $2$-set packing) problem is the design of an \emph{adaptive} algorithm that queries only a constant number of edges per vertex and achieves a $(1-\epsilon)$ fraction of the omniscient optimal solution, for an arbitrarily small $\epsilon>0$. Moreover, this adaptive algorithm performs the queries in only a constant number of rounds. We complement this result with a \emph{non-adaptive} (i.e., one round of queries) algorithm that achieves a $(0.5 - \epsilon)$ fraction of the omniscient optimum. We also extend both our results to stochastic $k$-set packing by designing an adaptive algorithm that achieves a $(\frac{2}{k} - \epsilon)$ fraction of the omniscient optimal solution, again with only $O(1)$ queries per element. This guarantee is close to the best known polynomial-time approximation ratio of $\frac{3}{k+1} -\epsilon$ for the \emph{deterministic} $k$-set packing problem [Furer and Yu, 2013] We empirically explore the application of (adaptations of) these algorithms to the kidney exchange problem, where patients with end-stage renal failure swap willing but incompatible donors. We show on both generated data and on real data from the first 169 match runs of the UNOS nationwide kidney exchange that even a very small number of non-adaptive edge queries per vertex results in large gains in expected successful matches.

==> introduction_kpd.tex <==
\section{Introduction}
\label{sec:intro}

%Our work is directly motivated by applications to kidney exchange, a medical approach that enables kidney transplants. Transplanted kidneys are usually harvested from deceased donors; but as of February \num{7}, \num{2015}, there are \num{101556} people on the US national waiting list\footnote{\url{http://optn.transplant.hrsa.gov}.}, making the median waiting time dangerously long. Fortunately, kidneys are an unusual organ in that donation by living donors is also a possibility---as long as patients happen to be medically compatible with their potential donors.

In kidney exchange, patients with inoperable kidney failure swap willing but incompatible donors.  In its simplest instantiation, pairwise kidney exchange, a patient's paired donor gives to a second patient, whose paired donor gives back to the first patient.  While logistically simple, pairwise kidney exchange leaves possible matches on the table~\cite{RSU07}; thus, fielded kidney exchanges typically permit more complicated swaps in larger \emph{cycles} or \emph{chains}, the latter of which is triggered by an altruistic donor who enters the exchange without a paired patient.  The kidney exchange problem is then to find the set of disjoint cycles and chains that results in the largest number of transplants.

Early models of kidney exchange did not take into account the possibility of an algorithmic match failing to result in an actual transplant.  In practice, this happens frequently~\cite{Leishman13:Organ}.  Due to logistical constraints, all transplants in a cycle must occur simultaneously, and a single match failure results in the cancellation of the entire cycle; thus, post-algorithmic match failure becomes more of a problem when exchanges allow complex matching structures---as fielded exchanges do.  %Thus, maximizing the cardinality of a match may not necessarily maximize the total number of transplants.

Formally, we can view an instance of the pairwise kidney exchange problem as a \emph{stochastic matching} problem on an undirected graph $G=(V,E)$, where we do not know which edges in $E$ actually exist. Rather, for each edge $e\in E$, we are given an existence probability $p_{e}$.  Similarly, we can view the general kidney exchange problem with cycles and chains up to length $k$ as a \emph{stochastic $k$-set packing} problem, where each set only exists probabilistically.  In both cases, we need to query edges or sets to find the ones that exist, and based on these queries, produce a matching or packing that is as large as possible.  Without any constraints, one can simply query all edges or sets, and then output the maximum matching or packing over those that exist.  However, in kidney exchange, such querying takes the form of a \emph{crossmatch test}, where the blood of a patient and potential donor is mixed in a laboratory---an expensive process in terms of money, time, and manpower.  Thus, constraining the number of such tests is preferred.

\citet{BGPS13} consider a stochastic matching setting with a budget of at most two crossmatches per vertex, and ask which subset of edges is queried by the optimal collection of queries subject to this constraint. They take an algorithmic viewpoint without establishing gains, and give a polynomial-time algorithm that finds an almost optimal solution on a class of random graphs (inspired by kidney exchange); crucially, their benchmark is also constrained to two queries per vertex. 


We ask: In order to perform as well as the omniscient optimum in the stochastic matching problem, do we need to query (almost) all the edges, that is, do our per-vertex budgets need to be $\Theta(n)$, where $n$ is the number of vertices? Or, can we, for any arbitrarily small $\epsilon>0$, achieve performance that is very close to the omniscient optimal solution by using an $o(n)$ per-vertex budget?  We answer this question, as well as its extension to the $k$-set packing problem.  We support our theoretical results empirically on both generated and real data from a large fielded kidney exchange in the United States.


\subsection{Our theoretical results and techniques}

Our main theoretical result gives a positive answer to the latter question for stochastic matching, by showing that, surprisingly, a \emph{constant} per-vertex budget is sufficient to get $\epsilon$-close to the omniscient optimum. Indeed, we design a polynomial-time algorithm with the following properties: for any constant $\epsilon>0$, the algorithm queries at most $O(1)$ edges incident to any particular vertex, requires $O(1)$ rounds of parallel queries, and achieves a $(1-\epsilon)$ fraction of the omniscient optimum.\footnote{This guarantee holds as long as all the non-zero $p_{e}$'s are bounded away from zero by some constant. The constant can be arbitrarily small but should not depend on $n$.} 

The foregoing algorithm is \emph{adaptive}, in the sense that its queries are conditioned on the answers to previous queries. Even though it requires only a constant number of rounds, it is natural to ask whether a non-adaptive algorithm---one that issues all its queries in one round---can also achieve a similar guarantee. We do not give a complete answer to this question, but we do present a non-adaptive algorithm that achieves a $0.5(1-\epsilon)$-approximation (for arbitrarily small $\epsilon>0$) to the omniscient optimum. We extend our matching results to a more general stochastic model in Appendix~\ref{sec:extensions}.

We extend our results to the stochastic $k$-set packing problem, where we are given a collection of sets, each with cardinality at most $k$. Stochastic Matching is a special case of Stochastic $k$-set packing: each set (which corresponds to an edge) has cardinality \num{2}, that is, $k=2$. In stochastic $k$-set packing, each set $s$ exists with some known probability $p_{s}$, and we need to query the sets to find whether they exist. Our objective is to output a collection of $\emph{disjoint}$ sets of maximum cardinality. 
We present adaptive and non-adaptive polynomial-time algorithms that achieve, for any constant $\epsilon>0$, at least $(\frac{2}{k}-\epsilon)$ and $(1-\epsilon)\frac{(2/k)^2}{2/k +1}$ fraction, respectively, of the omniscient optimum, again using $O(1)$ queries per element and hence $O(n)$ overall. For the sake of comparison, the best known \emph{polynomial-time} algorithm for optimizing $k$-set packing in the \emph{standard non-stochastic setting} has an approximation ratio of $\frac{3}{k+1} - \epsilon$~\citep{Furer:2013}. 

To better appreciate the challenge we face, we note that even in the stochastic matching setting, we do not have a clear idea of how large the omniscient optimum is. Indeed, there is a significant body of work on the expected cardinality of matching in \emph{complete} random graphs (see, e.g.,~\citep[Chapter 7]{Bol01}), where the omniscient optimum is known to be close to $n$. But in our work we are dealing with \emph{arbitrary} graphs where it can be a much smaller number. In addition, na\"ive algorithms fail to achieve our goal, even if they are allowed many queries. For example, querying a sublinear number of edges incident to each vertex, chosen uniformly at random, gives a vanishing fraction of the omniscient optimum---as we show in Section~\ref{sec:mod}. 

The primary technical ingredient in the design of our \emph{adaptive algorithm} is that if, in any round $r$ of the algorithm, the solution computed by round $r$ (based on previous queries) is small compared to the omniscient optimum, then the current structure must admit a \emph{large collection of disjoint constant-sized `augmenting' structures}. These augmenting structures are composed of sets that have not been queried so far. Of course, we do not know whether these structures we are counting on to help augment our current matching actually exist; but we do know that these augmenting structures have constant size (and so each structure exists with some constant probability) and are \emph{disjoint} (and therefore the outcomes of the queries to the different augmenting structures are independent). Hence, by querying all these structures in parallel in round $r$, in expectation, we can close a constant fraction of the gap between our current solution and the omniscient optimum. By repeating this argument over a constant number of rounds, we achieve a $(1-\epsilon)$ fraction of the omniscient optimum. In the case of stochastic matching, these augmenting structures are simply augmenting paths; in the more general case of $k$-set packing, we borrow the notion of augmenting structures from \citet{Hurkens:1989}. 

\subsection{Our experimental results: Application to kidney exchange}
\label{sec:kidney}
As discussed earlier, our work is directly motivated by applications to kidney exchange, a medical approach that enables kidney transplants. In its simplest form---\emph{pairwise exchange}---two incompatible donor-patient pairs exchange kidneys: the donor of the first pair donates to the patient of the second pair, and the donor of the second pair donates to the patient of the first pair.  This setting can be represented as an undirected \emph{compatibility graph}, where each vertex represents an incompatible donor-patient pair, and an edge between two vertices represents the possibility of a pairwise exchange. A matching in this graph specifies which exchanges take place. 

The edges of the compatibility graph can be determined based on the medical characteristics---blood type and tissue type---of donors and patients. However, the compatibility graph only tells part of the story. Before a transplant takes place, a more accurate medical test known as a \emph{crossmatch test} takes place. This test involves mixing samples of the blood of the patient and the donor (rather than simply looking up information in a database), making the test relatively costly and time consuming. Consequently, crossmatch tests are only performed for donors and patients that have been matched. While some patients are more likely to pass crossmatch tests than others---the probability is related to a measure of sensitization known as the person's Panel Reactive Antibody (PRA)---the average is as low as \num{30}\% in major kidney exchange programs~\citep{DPS13,Leishman13:Organ}. This means that, if we tested a perfect matching over $n$ donor-patient pairs, we would expect only $0.09n$ of the patients to actually receive a kidney. In contrast, the omniscient solution that runs crossmatch tests on all possible pairwise exchanges (in the compatibility graph) may be able to provide kidneys to all $n$ patients; but this solution is impractical.

Our adaptive algorithm for stochastic matching uncovers a sweet spot between these two extremes. On the one hand, it only mildly increases medical expenses, from one crossmatch test per patient, to a larger, yet constant, number; and it is highly parallelizable, requiring only a constant number of rounds, so the time required to complete all crossmatch tests does not scale with the number of donors and patients. On the other hand, the adaptive algorithm essentially recovers the entire benefit of testing all potentially feasible pairwise exchanges. To make policy recommendations, the next step must certainly involve extensive simulations; but the qualitative message of this theoretical result is clear: \emph{a mild increase in number of crossmatch tests provides nearly the full benefit of exhaustive testing.} 

The above discussion pertains to pairwise kidney exchange. However, modern kidney exchange programs regularly employ swaps involving three donor-patient pairs, which are known to provide significant benefit compared to pairwise swaps alone~\citep{RSU07,AR13}. Mathematically, we can consider a directed graph, where an edge $(u,v)$ means that the donor of pair $u$ is compatible with the patient of pair $v$ (before a crossmatch test was performed). In this graph, pairwise and \num{3}-way exchanges correspond to \num{2}-cycles and \num{3}-cycles, respectively. Our adaptive algorithm for \num{3}-set packing then provides a $(2/3)$-approximation to the omniscient optimum, using only $O(1)$ crossmatch tests per patient and $O(n)$ overall. While the practical implications of this result are currently not as crisp as those of its pairwise counterpart, future work may improve the approximation ratio (using $O(n)$ queries and an exponential-time algorithm), as we explain in Section~\ref{sec:conclusions-open}.

In this paper, we provide experiments on both simulated data and real data from the first \num{169} match runs of the United Network for Organ Sharing (UNOS) US nationwide kidney exchange, which now includes \num{143} transplant centers---approximatey \num{60}\% of the transplant centers in the US.  The exchange began matching in October 2010 and now matches on a biweekly basis.  Using adaptations of the algorithms presented in this paper, we show that even a small number of non-adaptive rounds, followed by a single period during which only those edges selected during those rounds are queried, results in large gains relative to the omniscient matching.  We discuss the policy implications of this promising result.


\section{Related work}
\label{sec:related-work}
Prior work has considered multiple variants of stochastic matching. A popular variant is the \emph{query-commit} problem, where the algorithm is \emph{forced} to add any queried edge to the matching if the edge is found to exist. In the papers of~\citet{GT12} and~\citet{CTT12}, lower bounds of \num{0.56} and \num{0.573}, respectively, and upper bounds of \num{0.7916} and \num{0.898}, respectively, are established for graphs in which no information is available about the edges, and in which each edge $e$ exists with a given probability $p_e$, respectively. Similarly to our work, these approximation ratios are with respect to the omniscient optimum, but the informational disadvantage of the algorithm stems purely from the query-commit restriction. 

Within the query-commit setting, another thread of work~\citep{CIKM+09,Adam11,BGLM+12} imposes an additional \emph{per-vertex budget constraint} where the algorithm is not allowed to query more than a specified number, $b_{v}$, of edges incident to vertex $v$. With this additional constraint, the benchmark that the algorithm is compared to switches from the omniscient optimum to the constrained optimum, i.e., the performance of the best decision tree that obeys the per-vertex budget constraints and the query-commit restriction. In other words, the algorithm's disadvantage compared to the benchmark is only that it is constrained to run in polynomial time. Here, again, the best known approximation ratios are constant. A generalization of these results to packing problems has been studied by~\citet{GN13}.

% Commented out because this is covered in the Introduction now
%Similarly to our work,~\citet{BGPS13} consider a stochastic matching setting without the query-commit constraint. They set the per-vertex budget to exactly $2$, and ask which subset of edges is queried by the optimal collection of queries subject to this constraint. They prove structural results about the optimal solution, which allow them to show that finding the optimal subset of edges to query is \textbf{NP}-hard. In addition, they give a polynomial-time algorithm that finds an almost optimal solution on a class of random graphs (inspired by kidney exchange settings). Crucially, the benchmark of~\citet{BGPS13} is also constrained to two queries per vertex. 

There is a significant body of work in stochastic optimization more broadly, for instance, the papers of \citet{Dean:2004} (Stochastic Knapsack), \citet{Gupta:2012} and \citet{Bansal:2014} (Stochastic Orienteering), and \citet{Asadpur:2008} (Stochastic submodular maximization).
 
Early models of kidney exchange did not explicitly consider the possibility of a modeled edge existing only probabilistically in reality.  Recent research by \citet{DPS13} and \citet{Anderson15:Finding} focuses on the kidney exchange application and restricts attention to a single crossmatch test per patient (the current practice), with a similar goal of maximizing the expected number of matched vertices, in a realistic setting (for example, they allow \num{3}-cycles and chains initiated by altruistic donors, who enter the exchange without a paired patient). They develop integer programming techniques, which are empirically evaluated using real and synthetic data.  \citet{Manlove15:Paired} discuss the integer programming formulation used by the national exchange in the United Kingdom, which takes edge failures into account in an ad hoc way by, for example, preferring shorter cycles to longer ones.  To our knowledge, our paper is the first to describe a general method for testing two or more edges \emph{before} the final match run is performed---and to provide experiments on real data showing the expected effect on fielded exchanges of such edge querying policies.
 
Another form of stochasticity present in fielded kidney exchanges is the arrival and departure of donor-patient pairs over time (and the associated arrival and departure of their involved edges in the compatibility graph).  Recent work has addressed this added form of dynamism from a theoretical~\cite{Unv10,Akbarpour14:Dynamic,Anderson15:Dynamic} and experimental~\cite{AS09,DPS12b,Dickerson15:FutureMatch} point of view.  Theoretical models have not addressed the case where an edge in the current graph may not exist (as we do in this paper); the more recent experimental papers have incorporated this possibility, but have not considered the problem of querying edges before recommending a final matching.  We leave as future research the analysis of edge querying in stochastic matching in such a dynamic model.

